Neural Rerendering in the Wild

We explore total scene capture -- recording, modeling, and rerendering a scene under varying appearance such as season and time of day. Starting from internet photos of a tourist landmark, we apply traditional 3D reconstruction to register the photos and approximate the scene as a point cloud. For each photo, we render the scene points into a deep framebuffer, and train a neural network to learn the mapping of these initial renderings to the actual photos. This rerendering network also takes as input a latent appearance vector and a semantic mask indicating the location of transient objects like pedestrians. The model is evaluated on several datasets of publicly available images spanning a broad range of illumination conditions. We create short videos demonstrating realistic manipulation of the image viewpoint, appearance, and semantic labeling. We also compare results with prior work on scene reconstruction from internet photos.

==> semantic_segmentations.tex <==
\begin{figure}[t]
    \captionsetup[subfigure]{aboveskip=1pt,belowskip=0pt}
    \centering
    \begin{subfigure}[b]{0.32\linewidth}
        \adjincludegraphics[width=\linewidth,trim={0 0 {.75\width} 0},clip]{figures_opt/segmentation/out_0025_gt.jpg}
        \caption{input render}
    \end{subfigure}\,%
    \begin{subfigure}[b]{0.66\linewidth}
        \adjincludegraphics[width=0.48\linewidth,trim={{.25\width} 0 {.5\width} 0},clip]{figures_opt/segmentation/out_0025_gt.jpg}\,%
        \adjincludegraphics[width=0.48\linewidth,trim={{.5\width} 0 {.25\width} 0},clip]{figures_opt/segmentation/out_0025_gt.jpg}\,%
        \caption{\footnotesize with ground-truth segmentation}
    \end{subfigure}\\
    \begin{subfigure}[b]{0.32\linewidth}
        \adjincludegraphics[width=\linewidth,trim={{.75\width} 0 0 0},clip]{figures_opt/segmentation/out_0025_gt.jpg}
        \caption{\footnotesize original image}
    \end{subfigure}\,%
    \begin{subfigure}[b]{0.66\linewidth}
        \adjincludegraphics[width=0.48\linewidth,trim={{.25\width} 0 {.5\width} 0},clip]{figures_opt/segmentation/out_0025_learnt.jpg}\,%
        \adjincludegraphics[width=0.48\linewidth,trim={{.5\width} 0 {.25\width} 0},clip]{figures_opt/segmentation/out_0025_learnt.jpg}\,%
        \caption{with learned segmentation}
    \end{subfigure}
    \caption{Example ground-truth semantic segmentation vs learned semantic segmentation and its effects on the rendering. Note the missing people detections in the learned segmentations, and how the pedestrians disappear from the rendering of the scene as well.}
    \label{fig:semantic_segmentation}
\end{figure}

